The Pseudo-Dimension of Contracts

Algorithmic contract design studies scenarios where a principal incentivizes an agent to exert effort on her behalf. In this work, we focus on settings where the agent's type is drawn from an unknown distribution, and formalize an offline learning framework for learning near-optimal contracts from sample agent types. A central tool in our analysis is the notion of pseudo-dimension from statistical learning theory. Beyond its role in establishing upper bounds on the sample complexity, pseudo-dimension measures the intrinsic complexity of a class of contracts, offering a new perspective on the tradeoffs between simplicity and optimality in contract design. Our main results provide essentially optimal tradeoffs between pseudo-dimension and representation error (defined as the loss in principal's utility) with respect to linear and bounded contracts. Using these tradeoffs, we derive sample- and time-efficient learning algorithms, and demonstrate their near-optimality by providing almost matching lower bounds on the sample complexity. Conversely, for unbounded contracts, we prove an impossibility result showing that no learning algorithm exists. Finally, we extend our techniques in three important ways. First, we provide refined pseudo-dimension and sample complexity guarantees for the combinatorial actions model, revealing a novel connection between the number of critical values and sample complexity. Second, we extend our results to menus of contracts, showing that their pseudo-dimension scales linearly with the menu size. Third, we adapt our algorithms to the online learning setting, where we show that, a polynomial number of type samples suffice to learn near-optimal bounded contracts. Combined with prior work, this establishes a formal separation between expert advice and bandit feedback for this setting.

==> commands.tex <==
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts     % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{booktabs} % for tables
\usepackage{etoolbox} % for tables
\usepackage{siunitx} % for tables
\sisetup{separate-uncertainty=true} % for tables
\usepackage{colortbl} % for tables


%\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{natbib}
%\usepackage{amssymb}
\usepackage{amsmath}
\definecolor{myblue}{rgb}{0.0, 0.0, 0.61}
\usepackage{graphicx}

\usepackage{float}
%\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{tikz}
\usetikzlibrary{matrix, shapes}

\usepackage{mathtools}
\usepackage{bbm}
\usepackage{tcolorbox}
\usepackage{cleveref}

\usepackage{wrapfig}

\newcommand{\phica}{\ensuremath{\phi^{\text{CA}}}}
\newrobustcmd{\ccell}{{\cellcolor{gray!40}}}

%%commands for preference generator
\usepackage{xcolor,colortbl}
\newcommand\E[1]{\mathbb{E}\left[#1\right]}
\newcommand{\D}{\mathcal{D}}
\newcommand{\clr}{\cellcolor{yellow}}
\newcommand\studentset[1]{N_{#1}}
\newcommand\student[0]{a}
\newcommand\courseset[1]{M_{#1}}
\newcommand\course[0]{m}
\newcommand\compset[1]{\mathbf{C}_{#1}}
\newcommand\ssubset[1]{\mathbf{S}_{#1}}
\newcommand{\ep}{\varepsilon}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{example}[theorem]{Example}


%commands for theoretical gaurantees
\newcommand{\ns}{\lvert N \rvert}
\newcommand{\x}{a}
\newcommand{\xii}{a_i}
\newcommand{\xij}{a_{ij}}
\newcommand{\xiis}{a^*_i}
\newcommand{\xijs}{a^*_{ij}}
\newcommand{\bb}{b}
\newcommand{\bp}{p}

%
\newcommand{\R}{\mathbb{R}}

% JAKOB W
\usepackage{amsmath}
\newrobustcmd{\crow}{{\rowcolor{gray!40}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}

\newcommand{\maximinshare}[2][]{
    \ensuremath{a^{\text{MaxiMin},#2,u_{#1}}} 
    }
\newcommand{\Epsmaximinshare}[3][]{
    \ensuremath{a^{\text{MaxiMin},(#2,#3),u_{#1}}} 
    }

\newcommand{\maximinsharehat}[2][]{
    \ensuremath{a^{\text{MaxiMin},#2,\hat{u}_{#1}}} 
    }
\newcommand{\Epsmaximinsharehat}[3][]{
    \ensuremath{a^{\text{MaxiMin},(#2,#3),\hat{u}_{#1}}} 
    }

==> figures/bounded_tradeoffs.tex <==
\begin{tikzpicture}[
    Deco/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=red}},
    Deco2/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=green}},
    scale=2.5
]

% First clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,0) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco] (0,0) rectangle (1.5,1);
\end{scope}

% Second clipped area
\begin{scope}
    \clip (1,0) -- (1,1) -- (1.5,1) -- (1.5,0) -- cycle;
    \fill[white] (0,0) rectangle (1.5,1);
\end{scope}

% Third clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,1.1) -- (0,1.1) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco2] (0,0) rectangle (2,2);
\end{scope}

% Axes
\draw[->] (-0.1,0) -- (1.7,0); % x-axis
\draw[->] (0,-0.1) -- (0,1.2); % y-axis

% Dashed lines
\draw[thin, dash pattern=on 1pt off 1pt] (0.3,0.75) -- (0.3,0);
\draw[thin, dash pattern=on 1pt off 0.5pt] (1,0.18) -- (1,0);

% Axis labels and markers
\node at (-0.27, 0.75) {$m \log n$};
\draw[-] (-0.05, 0.75) -- (0.05, 0.75);

\node at (0.3,-0.15) {$1/n$};
\draw (0.3,-0.05) -- (0.3,0.05);

\node at (1,-0.15) {$\Theta(1/m^2)$};
\draw (1,-0.05) -- (1,0.05);

\node at (1.7, -0.15) {$\text{rep. error } \epsilon$};
\node at (-0.26, 1.27) {{pseudo-dim}};

% Curves and lines
\draw[-, green!80!black, line width=1pt] (0,0.75) -- (0.3,0.75);
\draw[green!80!black, line width=1pt] (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1);

% Log label
\node[scale=0.8, fill=white, inner sep=2pt] at (1, 0.4) {$m \log(1/\epsilon)$};
\draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=0.6pt] (0.95, 0.33) -- (0.88, 0.25);

% First sub-image
\begin{scope}[shift={(0.2, 0.95)}, scale=0.4]
    \draw[->] (-0.1,0) -- (1.2,0);
    \draw[->] (0,-0.1) -- (0,1.2);
    \fill[orange!20] (0,0) rectangle (1,1);

    \foreach \x/\label in {0/{0}, 1/{1}} {
        \draw[black] (\x, -0.1) -- (\x, 0.1);
        \node[scale=0.5] at (\x, -0.2) {${\label}$};
    }
    \foreach \y/\label in {0/{0}, 1/{1}} {
        \draw[black] (-0.1, \y) -- (0.1, \y);
        \node[scale=0.5] at (-0.2, \y) {${\label}$};
    }
    \draw[-,orange] (0,0) rectangle (1,1);
\end{scope}

% Second sub-image
\begin{scope}[shift={(0.8, 0.625)}, scale=0.4]
    \draw[->] (-0.1,0) -- (1.2,0);
    \draw[->] (0,-0.1) -- (0,1.2);
    \fill[white] (0,0) rectangle (1,1);

    \foreach \x/\label in {0/{0}, 1/{1}} {
        \draw[black] (\x, -0.1) -- (\x, 0.1);
        \node[scale=0.5] at (\x, -0.2) {${\label}$};
    }
    \foreach \y/\label in {0/{0}, 1/{1}} {
        \draw[black] (-0.1, \y) -- (0.1, \y);
        \node[scale=0.5] at (-0.2, \y) {${\label}$};
    }
    \draw[] (0,0) rectangle (1,1);

    \filldraw (1, 1) circle (0.015);

    % Orange dots
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 1.0 / 5.0, 1 - \x * 0 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 0.9848 / 5.0, 1 - \x * 0.1736 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 0.9397 / 5.0, 1 - \x * 0.3420 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3} {
        \filldraw[orange] (1 - \x * 0.8660 / 5.0, 1 - \x * 0.5000 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3, 18/3} {
        \filldraw[orange] (1 - \x * 0.7660 / 5.0, 1 - \x * 0.6428 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3, 18/3} {
        \filldraw[orange] (1 - \x * 0.6428 / 5.0, 1 - \x * 0.7660 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3} {
        \filldraw[orange] (1 - \x * 0.5000 / 5.0, 1 - \x * 0.8660 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 0.3420 / 5.0, 1 - \x * 0.9397 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 0.1736 / 5.0, 1 - \x * 0.9848 / 5.0) circle (0.015);
    }
    
    \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
        \filldraw[orange] (1 - \x * 0 / 5.0, 1 - \x * 1 / 5.0) circle (0.015);
    }
\end{scope}

% Third sub-image
\begin{scope}[shift={(1.4, 0.3)}, scale=0.4]
    \draw[->] (-0.1,0) -- (1.2,0);
    \draw[->] (0,-0.1) -- (0,1.2);
    \fill[white] (0,0) rectangle (1,1);

    \foreach \x/\label in {0/{0}, 1/{1}} {
        \draw[black] (\x, -0.1) -- (\x, 0.1);
        \node[scale=0.5] at (\x, -0.2) {$\label$};
    }
    \foreach \y/\label in {0/{0}, 1/{1}} {
        \draw[black] (-0.1, \y) -- (0.1, \y);
        \node[scale=0.5] at (-0.2, \y) {$\label$};
    }
    \draw[] (0,0) rectangle (1,1);

    \filldraw (1,1) circle (0.4*0.025);

    \foreach \x in {0,1,2,3,4,5} {
        \filldraw[orange] (1-\x*1.0/5.0, 1-\x*0/5.0) circle (0.015);
    }
    
    \foreach \x in {0,1,2,3,4,5} {
        \filldraw[orange] (1-\x*0.95/5.0, 1-\x*0.30/5.0) circle (0.015);
    }
    
    \foreach \x in {0,1,2,3,4,5,6} {
        \filldraw[orange] (1-\x*0.80/5.0, 1-\x*0.58/5.0) circle (0.015);
    }
    
    \foreach \x in {0,1,2,3,4,5,6} {
        \filldraw[orange] (1-\x*0.58/5.0, 1-\x*0.80/5.0) circle (0.015);
    }
    
    \foreach \x in {0,1,2,3,4,5} {
        \filldraw[orange] (1-\x*0.30/5.0, 1-\x*0.95/5.0) circle (0.015);
    }
    
    \foreach \x in {0,1,2,3,4,5} {
        \filldraw[orange] (1-\x*0/5.0, 1-\x*1/5.0) circle (0.015);
    }
\end{scope}

\end{tikzpicture}


==> figures/bounded_tradeoffs_2.tex <==
\begin{tikzpicture}[
    Deco/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=red}},
    Deco2/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=green}},
    scale=2.5
]

% First clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,0) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco] (0,0) rectangle (1.5,1);
\end{scope}

% Second clipped area
\begin{scope}
    \clip (1,0) -- (1,1) -- (1.5,1) -- (1.5,0) -- cycle;
    \fill[white] (0,0) rectangle (1.5,1);
\end{scope}

% Third clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,1.1) -- (0,1.1) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco2] (0,0) rectangle (2,2);
\end{scope}

% Axes
\draw[->] (-0.1,0) -- (1.7,0); % x-axis
\draw[->] (0,-0.1) -- (0,1.2); % y-axis

% Dashed lines
\draw[thin, dash pattern=on 1pt off 1pt] (0.3,0.75) -- (0.3,0);
\draw[thin, dash pattern=on 1pt off 0.5pt] (1,0.18) -- (1,0);

% Axis labels and markers
\node at (-0.27, 0.75) {$m \log n$};
\draw[-] (-0.05, 0.75) -- (0.05, 0.75);

\node at (0.3,-0.15) {$1/n$};
\draw (0.3,-0.05) -- (0.3,0.05);

\node at (1,-0.15) {$\Theta(1/m^2)$};
\draw (1,-0.05) -- (1,0.05);

\node at (1.7, -0.15) {$\text{rep. error } \epsilon$};
\node at (0.25, 1.27) {{pseudo-dimension}};

% Curves and lines
\draw[-, green!80!black, line width=1pt] (0,0.75) -- (0.3,0.75);
\draw[green!80!black, line width=1pt] (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1);

% Log label
\node[scale=0.8, fill=white, inner sep=2pt] at (1, 0.45) {$\tilde{\Theta}(m \log(1/\epsilon))$};
\draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=0.6pt] (0.95, 0.35) -- (0.88, 0.25);

% First sub-image
% \begin{scope}[shift={(0.2, 0.95)}, scale=0.4]
%     \draw[->] (-0.1,0) -- (1.2,0);
%     \draw[->] (0,-0.1) -- (0,1.2);
%     \fill[orange!20] (0,0) rectangle (1,1);

%     \foreach \x/\label in {0/{0}, 1/{1}} {
%         \draw[black] (\x, -0.1) -- (\x, 0.1);
%         \node[scale=0.5] at (\x, -0.2) {${\label}$};
%     }
%     \foreach \y/\label in {0/{0}, 1/{1}} {
%         \draw[black] (-0.1, \y) -- (0.1, \y);
%         \node[scale=0.5] at (-0.2, \y) {${\label}$};
%     }
%     \draw[-,orange] (0,0) rectangle (1,1);
% \end{scope}

% Second sub-image
% \begin{scope}[shift={(0.8, 0.625)}, scale=0.4]
%     \draw[->] (-0.1,0) -- (1.2,0);
%     \draw[->] (0,-0.1) -- (0,1.2);
%     \fill[white] (0,0) rectangle (1,1);

%     \foreach \x/\label in {0/{0}, 1/{1}} {
%         \draw[black] (\x, -0.1) -- (\x, 0.1);
%         \node[scale=0.5] at (\x, -0.2) {${\label}$};
%     }
%     \foreach \y/\label in {0/{0}, 1/{1}} {
%         \draw[black] (-0.1, \y) -- (0.1, \y);
%         \node[scale=0.5] at (-0.2, \y) {${\label}$};
%     }
%     \draw[] (0,0) rectangle (1,1);

%     \filldraw (1, 1) circle (0.015);

%     % Orange dots
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 1.0 / 5.0, 1 - \x * 0 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 0.9848 / 5.0, 1 - \x * 0.1736 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 0.9397 / 5.0, 1 - \x * 0.3420 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3} {
%         \filldraw[orange] (1 - \x * 0.8660 / 5.0, 1 - \x * 0.5000 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3, 18/3} {
%         \filldraw[orange] (1 - \x * 0.7660 / 5.0, 1 - \x * 0.6428 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3, 18/3} {
%         \filldraw[orange] (1 - \x * 0.6428 / 5.0, 1 - \x * 0.7660 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3, 16/3} {
%         \filldraw[orange] (1 - \x * 0.5000 / 5.0, 1 - \x * 0.8660 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 0.3420 / 5.0, 1 - \x * 0.9397 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 0.1736 / 5.0, 1 - \x * 0.9848 / 5.0) circle (0.015);
%     }
    
%     \foreach \x in {0, 2/3, 4/3, 6/3, 8/3, 10/3, 12/3, 14/3} {
%         \filldraw[orange] (1 - \x * 0 / 5.0, 1 - \x * 1 / 5.0) circle (0.015);
%     }
% \end{scope}

% Third sub-image
% \begin{scope}[shift={(1.4, 0.3)}, scale=0.4]
%     \draw[->] (-0.1,0) -- (1.2,0);
%     \draw[->] (0,-0.1) -- (0,1.2);
%     \fill[white] (0,0) rectangle (1,1);

%     \foreach \x/\label in {0/{0}, 1/{1}} {
%         \draw[black] (\x, -0.1) -- (\x, 0.1);
%         \node[scale=0.5] at (\x, -0.2) {$\label$};
%     }
%     \foreach \y/\label in {0/{0}, 1/{1}} {
%         \draw[black] (-0.1, \y) -- (0.1, \y);
%         \node[scale=0.5] at (-0.2, \y) {$\label$};
%     }
%     \draw[] (0,0) rectangle (1,1);

%     \filldraw (1,1) circle (0.4*0.025);

%     \foreach \x in {0,1,2,3,4,5} {
%         \filldraw[orange] (1-\x*1.0/5.0, 1-\x*0/5.0) circle (0.015);
%     }
    
%     \foreach \x in {0,1,2,3,4,5} {
%         \filldraw[orange] (1-\x*0.95/5.0, 1-\x*0.30/5.0) circle (0.015);
%     }
    
%     \foreach \x in {0,1,2,3,4,5,6} {
%         \filldraw[orange] (1-\x*0.80/5.0, 1-\x*0.58/5.0) circle (0.015);
%     }
    
%     \foreach \x in {0,1,2,3,4,5,6} {
%         \filldraw[orange] (1-\x*0.58/5.0, 1-\x*0.80/5.0) circle (0.015);
%     }
    
%     \foreach \x in {0,1,2,3,4,5} {
%         \filldraw[orange] (1-\x*0.30/5.0, 1-\x*0.95/5.0) circle (0.015);
%     }
    
%     \foreach \x in {0,1,2,3,4,5} {
%         \filldraw[orange] (1-\x*0/5.0, 1-\x*1/5.0) circle (0.015);
%     }
% \end{scope}

\end{tikzpicture}


==> figures/linear_tradeoffs.tex <==
\begin{tikzpicture}[
    Deco/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=red}},
    Deco2/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=green}},
    scale=2.5
]

% First clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,0) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco] (0,0) rectangle (1.5,1);
\end{scope}

% Second clipped area
% \begin{scope}
%     \clip (1,0) -- (1,1) -- (1.5,1) -- (1.5,0) -- cycle;
%     \fill[white] (0,0) rectangle (1.5,1);
% \end{scope}

% Third clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,1.1) -- (0,1.1) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco2] (0,0) rectangle (2,2);
\end{scope}

% Axes
\draw[->] (-0.1,0) -- (1.7,0); % x-axis
\draw[->] (0,-0.1) -- (0,1.2); % y-axis

% Dashed lines
\draw[thin, dash pattern=on 1pt off 1pt] (0.3,0.75) -- (0.3,0);
% \draw[thin, dash pattern=on 1pt off 0.5pt] (1,0.18) -- (1,0);

% Axis labels and markers
\node at (-0.22, 0.75) {$\log n$};
\draw[-] (-0.05, 0.75) -- (0.05, 0.75);

\node at (0.3,-0.15) {$1/n$};
\draw (0.3,-0.05) -- (0.3,0.05);

% \node at (1,-0.15) {$\Theta(1/m^2)$};
% \draw (1,-0.05) -- (1,0.05);

\node at (1.7, -0.15) {$\text{rep. error } \epsilon$};
\node at (-0.26, 1.27) {{pseudo-dim}};

% Curves and lines
\draw[-, green!80!black, line width=1pt] (0,0.75) -- (0.3,0.75);
\draw[green!80!black, line width=1pt] (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1);

% Log label
\node[scale=0.8, fill=white, inner sep=2pt] at (1, 0.4) {$\log(1/\epsilon)$};
\draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=0.6pt] (0.95, 0.33) -- (0.88, 0.25);

% First sub-image
    \begin{scope}[shift={(0.2, 0.95)}, scale=0.4, fill=white] % Adjust scale to make it smaller
    \fill[white] (-0.2,-0.3) -- (1.2,-0.3) -- (1.2,0.2) -- (-0.2,0.2);
    
        % Draw x-axis arrow (without label)
        \draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=1pt] (-0.2,0) -- (1.2,0);

        % Draw black vertical ticks and labels
        \draw[black] (0, -0.1) -- (0, 0.1);
        \draw[black] (1, -0.1) -- (1, 0.1);

        % Label points 0 and 1
        \node[scale=0.5] at (0, -0.25) { $0$ };
        \node[scale=0.5] at (1, -0.25) { $1$ };

        % Label contract space and interval
        % \node[scale=0.4*0.3] at (0.5, -0.15) {$\bm{\mathcal{C}_{\mathrm{linear}} = [0,1]}$};
        % \node[scale = 0.4*0.3] at (0.5, 0.15) {\textbf{contract space}};

        % Red line for the interval [0,1]
        \draw[red, line width=1.5pt] (0,0) -- (1,0);
    \end{scope}


% Second sub-image
\begin{scope}[shift={(0.8, 0.625)}, scale=0.4]
    \fill[white] (-0.2,-0.2) -- (1.2,-0.2) -- (1.2,0.2) -- (-0.2,0.2);
    % Adjust scale to make it smaller
        % Draw x-axis arrow (without label)
        \draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=1pt] (-0.2,0) -- (1.2,0);

     

        % Black lines at the start and end
        \draw[black] (0, -0.1) -- (0, 0.1);
        \draw[black] (1, -0.1) -- (1, 0.1);
    
        % Dense tick marks
        \foreach \x in {0, 0.0625, 0.125, 0.1875, 0.25, 0.3125, 0.375, 0.4375, 0.5, 0.5625, 0.625, 0.6875, 0.75, 0.8125, 0.875, 0.9375, 1} {
            \draw[red, line width=0.75pt] (\x, -0.05) -- (\x, 0.05); % Small, dense ticks
        }
    \end{scope}

% Third sub-image
\begin{scope}[shift={(1.4, 0.3)}, scale=0.4] % Adjust scale to make it smaller
    \fill[white] (-0.2,-0.2) -- (1.2,-0.2) -- (1.2,0.2) -- (-0.2,0.2);
        % Draw x-axis arrow (without label)
        \draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=1pt] (-0.2,0) -- (1.2,0);

       \draw[black] (0, -0.1) -- (0, 0.1);

        \draw[black] (1, -0.1) -- (1, 0.1);
        
        % Mark points 0, 1/8, 2/8, 1 with small vertical lines and green marks
        \foreach \x/\label in {0/{0}, 0.125/{\frac{1}{\epsilon}}, 0.250/{\frac{2}{\epsilon}}, 0.375/{}, 0.5/{\ldots}, 0.625/{}, 0.75/{}, 0.875/{}, 1/{1}} {
            \draw[red, line width=1pt] (\x, -0.05) -- (\x, 0.05); % green marks at each point
        }
    \end{scope}

\end{tikzpicture}


==> figures/linear_tradeoffs_2.tex <==
\begin{tikzpicture}[
    Deco/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=red}},
    Deco2/.style={postaction={pattern={Lines[angle=45, distance=0.2mm, line width=0.1mm]}, pattern color=green}},
    scale=2.5
]

% First clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,0) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco] (0,0) rectangle (1.5,1);
\end{scope}

% Second clipped area
% \begin{scope}
%     \clip (1,0) -- (1,1) -- (1.5,1) -- (1.5,0) -- cycle;
%     \fill[white] (0,0) rectangle (1.5,1);
% \end{scope}

% Third clipped area
\begin{scope}
    \clip (0,0.75) -- (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1) -- (1.5,1.1) -- (0,1.1) -- (0,0) -- cycle;
    \fill[pattern=north east lines, pattern color=white, Deco2] (0,0) rectangle (2,2);
\end{scope}

% Axes
\draw[->] (-0.1,0) -- (1.7,0); % x-axis
\draw[->] (0,-0.1) -- (0,1.2); % y-axis

% Dashed lines
\draw[thin, dash pattern=on 1pt off 1pt] (0.3,0.75) -- (0.3,0);
% \draw[thin, dash pattern=on 1pt off 0.5pt] (1,0.18) -- (1,0);

% Axis labels and markers
\node at (-0.22, 0.75) {$\log n$};
\draw[-] (-0.05, 0.75) -- (0.05, 0.75);

\node at (0.3,-0.15) {$1/n$};
\draw (0.3,-0.05) -- (0.3,0.05);

% \node at (1,-0.15) {$\Theta(1/m^2)$};
% \draw (1,-0.05) -- (1,0.05);

\node at (1.7, -0.15) {$\text{rep. error } \epsilon$};
\node at (0.25, 1.27) {{pseudo-dimension}};

% Curves and lines
\draw[-, green!80!black, line width=1pt] (0,0.75) -- (0.3,0.75);
\draw[green!80!black, line width=1pt] (0.3,0.75) .. controls (0.4,0.4) and (0.7,0.2) .. (1.5,0.1);

% Log label
\node[scale=0.8, fill=white, inner sep=2pt] at (1, 0.45) {$\tilde{\Theta}(\log(1/\epsilon))$};
\draw[->, >={Latex[length=1pt, width=1.3pt]}, line width=0.6pt] (0.95, 0.35) -- (0.88, 0.25);

\end{tikzpicture}


==> figures/tradeoffs.tex <==
\newcommand{\overn}{0.25}
\newcommand{\mlogn}{0.55*ln(1/\overn)}
\newcommand{\logn}{0.4*ln(1/\overn)}
\newcommand{\overm}{0.5}
\begin{figure}[t]
    \centering
    % Two subfigures
    \subfloat[Pareto frontier for linear contracts.]{
        \centering
        \begin{tikzpicture}
        \begin{axis}[
          width=\textwidth, height=\textwidth,
          clip = false,
          xtick={0},
          ytick={0},
          xticklabels = {$0$},
          yticklabels = {$0$},
          %xlabel={representation error $\epsilon$},
          ylabel={pseudo-dimension $d$},
          %xlabel style={at={(axis description cs:0,0.75)}},
          ylabel style={at={(axis description cs:0,0.3)}},
          xmin=0,  xmax=1, ymin=0,  ymax=1, scale=0.46]
          \addplot [name path=straight,domain=0:\overn] {\logn};
          \addplot [name path=curved,domain=\overn:1] {0.4*ln(1/x)};
          \path[name path=topaxis] (axis cs:0,1) -- (axis cs:1,1);
          \path[name path=botaxis] (axis cs:0,0) -- (axis cs:1,0);
          \begin{scope}
            \clip (\overn,0) rectangle (1,1); 
            \tikzfillbetween[of=curved and botaxis,on layer=main] {pattern=north east lines};
          \end{scope}
          \begin{scope}
            \clip (0,0) rectangle (\overn,1); 
            \tikzfillbetween[of=straight and botaxis, on layer=main] {pattern=north east lines};
          \end{scope}
          \begin{scope}
            \clip (\overn,0) rectangle (1,1); 
            \tikzfillbetween[of=topaxis and curved,on layer=background] {black!5!white};
          \end{scope}
          \begin{scope}
            \clip (0,0) rectangle (\overn,1); 
            \tikzfillbetween[of=topaxis and straight,on layer=background] {black!5!white};
          \end{scope}
          %% HERE 
          %% \draw[dotted,thick] (\overn,0) -- (\overn,\logn);
          \draw[dotted,thick] (0.25,0) -- (0.25,0.5545177);
          \node[fill=white] at (0.25,0.15) {non-existence};
          \fill[white] (0.33,0.71) rectangle (0.97,0.93);
          \node at (0.65,0.89) {\small existence of a contract class};
          \node at (0.65,0.82) {\small with representation error $\epsilon$};
          \node at (0.65,0.75) {\small and pseudo-dimension $d$};
          \node[anchor=north,fill=white] (overeps) at (0.6,0.45) {${\Theta}(\log(1/\epsilon))$};
          \draw[->] (overeps) to (0.55,0.25);
          \node[anchor=north,fill=white] (overn) at (0.15,0.7) {${\Theta}(\log n)$};
          \draw[->] (overn) to (0.15,0.57);
          \node at (0.87, -0.05) { rep. error $\epsilon$ };
          \node at (0.87, -0.11) { w.r.t. $\mathcal{C}_{\text{linear}}$};
          \node at (\overn, -0.05) {$1/n$};
        \end{axis}
        \end{tikzpicture}
        \label{fig:linear_tradeoffs}
    }
    \hfill
    \subfloat[Pareto frontier for bounded contracts.]{
        \centering
        \begin{tikzpicture}
        \begin{axis}[
          width=\textwidth, height=\textwidth,
          clip = false,
          xtick={0},
          ytick={0},
          xticklabels = {$0$},
          yticklabels = {$0$},
          %xlabel={representation error $\epsilon$},
          ylabel={pseudo-dimension $d$},
          %xlabel style={at={(axis description cs:0.75,0)}},
          ylabel style={at={(axis description cs:0,0.3)}},
          xmin=0,  xmax=1, ymin=0,  ymax=1,scale=0.46]
          \addplot [name path=straight,domain=0:\overn] {\mlogn};
          \addplot [name path=curved,domain=\overn:1] {0.55*ln(1/x)};
          \path[name path=topaxis] (axis cs:0,1) -- (axis cs:1,1);
          \path[name path=botaxis] (axis cs:0,0) -- (axis cs:1,0);
          \begin{scope}
            \clip (\overn,0) rectangle (\overm,1); 
            \tikzfillbetween[of=curved and botaxis,on layer=main] {pattern=north east lines};
          \end{scope}
          \begin{scope}
            \clip (0,0) rectangle (\overn,1); 
            \tikzfillbetween[of=straight and botaxis, on layer=main] {pattern=north east lines};
          \end{scope}
          \begin{scope}
            \clip (\overn,0) rectangle (1,1); 
            \tikzfillbetween[of=topaxis and curved,on layer=background] {black!5!white};
          \end{scope}
          \begin{scope}
            \clip (0,0) rectangle (\overn,1); 
            \tikzfillbetween[of=topaxis and straight,on layer=background] {black!5!white};
          \end{scope}
          %% HERE
          %\draw[dotted,thick] (\overn,0) -- (\overn,\mlogn);
          \draw[dotted,thick] (0.25,0) -- (0.25,0.76246189);
          %% HERE 
          %\draw (\overm,0) -- (\overm,0.55*ln(1/\overm)); 
          \draw (0.5,0) -- (0.5,0.3812309); 
          \node[fill=white] at (0.25,0.15) {non-existence};
          \fill[white] (0.33,0.71) rectangle (0.97,0.93);
          \node at (0.65,0.89) {\small existence of a contract class};
          \node at (0.65,0.82) {\small with representation error $\epsilon$};
          \node at (0.65,0.75) {\small and pseudo-dimension $d$};
          \node[anchor=north,fill=white] (overeps) at (0.65,0.6) {$\widetilde{\Theta}(m \log(1/\epsilon))$};
          \draw[->] (overeps) to (0.46,0.45);
          \node[anchor=north,fill=white] (overn) at (0.16,0.93) {$\widetilde{\Theta}(m \log n)$};
          \draw[->] (overn) to (0.16,0.77);
          \node at (0.87, -0.05) { rep. error $\epsilon$ };
          \node at (0.87, -0.11) { w.r.t. $\mathcal{C}_{\text{bounded}}$};
          \node at (0.65, 0.1) { ? };
          \node at (\overn, -0.05) {$1/n$};
          \node at (\overm, -0.05) {$\Theta(1/m^2)$};
        \end{axis}
        \end{tikzpicture}
        \label{fig:bounded_tradeoffs}
    }
\caption{Trade-offs between pseudo-dimension and representation error for linear and bounded contracts in the case where $n > 24 \cdot m^2$.
For every point $(\epsilon,d)$, an $\epsilon$-approximation with pseudo-dimension $d$ exists if $(\epsilon,d)$ is in the gray region, and it does not exist if $(\epsilon,d)$ is in the diagonally-marked region.
For clarity, we suppress the logarithmic factors in this figure. Specifically, the boundaries between the two regions are tight up to a constant for linear contracts and up to a factor of $\log m$ for bounded contracts.
}
    \label{fig:tradeoffs_summary}
\end{figure}


==> tradeoffs_table_ec.tex <==
\begin{table}[t]
%\vspace{-1cm}
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Contract Class} & \multicolumn{2}{c|}{\textbf{Pseudo-Dimension}} & \textbf{Sample Complexity} \\ 
    % & Representation Error & Representation Error & \\ 
    \hline 
    % & Representation Error & Representation Error & \\ 
    & \textbf{Full Class} & \textbf{$\bm{\epsilon}$-Approximation} & \\ 
    \hline%\cmidrule{1-4}
    $\mathcal{C}_{\mathrm{linear}} = \{\alpha \cdot r : \alpha \in [0,1]\}$ & $\Theta(\log n)$ & ${\Theta}(\log (1/\epsilon))$ & ${\widetilde{\Theta}((1/\epsilon^2) \log (1/\delta))}$ \\
     & {\footnotesize (\Cref{theorem:linear_contract_pdim,theorem:special_case})} & {\footnotesize(\Cref{theorem:t_contracts_true_pd,thm:pdim_lb_for_rep_error_eps})} & {\footnotesize(\Cref{thm:efficient_linear,thm:sample_lower_bound_linear})} \\ \hline
    $\Cbounded = [0,1]^m$ & $\widetilde{\Theta}(m \log n)$ & $\widetilde{\Theta}(m \log (1/\epsilon))$ & $\widetilde{\Theta} ((1/\epsilon^2)(m + \log(1/\delta))$ \\
     & {\footnotesize (\Cref{theorem:general_contract_pdim,theorem:special_case})} & {\footnotesize(\Cref{lemma:se_contracts_pseudo-dimension,thm:pdim_lb_for_rep_error_eps})} & {\footnotesize(\Cref{thm:cone_efficient,thm:sample_complexity_lb_bounded_contracts})} \\ \hline
    $\Cunbounded = [0, \infty)^m$ & $\widetilde{\Theta}(m \log n)$ & - & $\infty$ \\
     & {\footnotesize(\Cref{theorem:general_contract_pdim,theorem:special_case})} & - & {\footnotesize(\Cref{thm:sample_impossibility_unbounded_contracts})} \\ \hline
    \end{tabular}
    \caption{Overview of our upper and lower bounds on the pseudo-dimension and sample complexity of key classes of contracts. Here, the $\widetilde{\Theta}$ notation suppresses {the $\log(1/\epsilon)$ and $\log m$ factors in the bounds that already depend polynomially on $1/\epsilon$ and $m$, respectively. 
    The pseudo-dimension lower bounds hold for any $\epsilon$-approximation of the corresponding full contract class. 
    }
    }
    \label{tab:overview}
\end{table}


